Acquisition of Spatially-Varying Reflectance and Surface Normals via Polarized Reflectance Fields

Accurately measuring the geometry and spatially-varying reflectance of real-world objects is a complex task due to their intricate shapes formed by concave features, hollow engravings and diverse surfaces, resulting in inter-reflection and occlusion when photographed. Moreover, issues like lens flare and overexposure can arise from interference from secondary reflections and limitations of hardware even in professional studios. In this paper, we propose a novel approach using polarized reflectance field capture and a comprehensive statistical analysis algorithm to obtain highly accurate surface normals (within 0.1mm/px) and spatially-varying reflectance data, including albedo, specular separation, roughness, and anisotropy parameters for realistic rendering and analysis. Our algorithm removes image artifacts via analytical modeling and further employs both an initial step and an optimization step computed on the whole image collection to further enhance the precision of per-pixel surface reflectance and normal measurement. We showcase the captured shapes and reflectance of diverse objects with a wide material range, spanning from highly diffuse to highly glossy - a challenge unaddressed by prior techniques. Our approach enhances downstream applications by offering precise measurements for realistic rendering and provides a valuable training dataset for emerging research in inverse rendering. We will release the polarized reflectance fields of several captured objects with this work.

==> fig/tab/Memory.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{cccc}
        \hline
         Cost&  Raw&  Storage& Runtime\\
         \hline
         Single Image&  -&  114.01 MB& 227.81 MB\\
         OLAT&  2.99 GB&  28.53 GB& 76.97 GB\\
         Full Scan&  47.85 GB&  616.33 GB& -\\
         \hline
 Format& R3D& OpenEXR&-\\
         \hline
    \end{tabular}
    \caption{Storage and Memory Cost. The cost is measured on a per-scan basis.}
    \label{tab:storage_and_memory}
\end{table}
% \vspace{-20pt}

==> fig/tex/Ablation.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{fig/jpg/Rendering Ablation.jpg}
    \vspace{-20pt}
    \caption{\textbf{Renderings with Various Material Components} We evaluate the rendering quality by comparing renderings against the f) captured image progressively, starting from a) only utilizing $\hat{\rho}_d$, b) then including $\hat{n}_d$, $\hat{n}_s$, followed by the incorporation of c) $\gamma$, and considering d) $\hat{\rho}_s$, and finally e) $\varsigma$.
    % \yajie{It's really confusing, you should use a b c d e f instead of repeating (a) and (b). Also what are each pairs?}
    % $\hat{\rho}_d$, $\hat{\rho}_s$, $\varsigma$, $\hat{n}_d$, $\hat{n}_s$, $\gamma$
    }
    \label{fig:ablation_relighting}
    \vspace{-15pt}
\end{figure*}

==> fig/tex/Cmp_Renderings.tex <==
\begin{figure}[t]
    \centering
    \vspace{-20pt}
    \includegraphics[width=\linewidth]{fig/jpg/Cmp Rendering.jpg}
    \vspace{-22pt}
    \caption{\textbf{Rendering Comparisons}. We compare a) ground truth captures with b) rendering results using c) the measured materials (upper left to bottom right: $\hat{\rho}_d$, $\hat{\rho}_s$, $\varsigma$, $\hat{n}_d$, $\hat{n}_s$, $\gamma$).}
    % \vspace{-20pt}
    \label{fig:cmp_renderings}
\end{figure}
% https://docs.google.com/presentation/d/122Q1jpwf4hr1TJ3LwoFOMYoKReKFVEb-lpQLtBW_gXs/edit?usp=sharing

==> fig/tex/Gradient_Synthesis.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-20pt}
    \includegraphics[width=\linewidth]{fig/jpg/Gradient Synthesis.jpg}
    % \vspace{-23pt}
    \caption{\textbf{Gradient Illumination Synthesis.} We present the synthesized gradient illumination in the x, y, and z directions, labeled as a), b), and c) respectively. Row 1) illustrates the lighting weight map. These maps are generated via equirectangular projection from the light's location, with intensity values representing the weights. Rows 2) and 3) showcase the synthesis under the cross and parallel polarization respectively. The smaller view in the lower-left corner highlights the value in red (\textcolor{red}{-}) and green (\textcolor{green}{+}).}
    % \vspace{-10pt}
    \label{fig:gradient_synthesis}
\end{figure}
% https://docs.google.com/presentation/d/1A58ywBp7hytsvQdanppqEkaocVKMvCwF_wJVpUBIblM/edit?usp=sharing

==> fig/tex/Supp_Qualitative.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/jpg/Supp_Qualitative.jpg}
    \caption{\textbf{More Optimization Results.} We present a wooden painted cube from a) left and b) right, a fabric bag from c) right and d) front, and a gift box from e) left and f) right. For each object, we showcase 1) original image, 2) diffuse albedo $\hat{\rho}_d$, 3) specular albedo $\hat{\rho}_s$, 4) diffuse normal $\hat{n}_d$, 5) specular normal $\hat{n}_s$, 6) anisotropy $\varrho$, and 7) roughness $\gamma$.}
    \label{fig:supp_qualitative}
\end{figure*}
% https://docs.google.com/presentation/d/1MHPsaoRJKB4KSRbejoh7Y48wnkHT3NY7Jn2bLGdH2VA/edit?usp=sharing

==> fig/tex/Visibility_Improvements.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-20pt}
    \includegraphics[width=\linewidth]{fig/jpg/Visibility_Improvements.jpg}
    \vspace{-20pt}
    \caption{\textbf{Improvements with Visibility.} We present a comparison of optimization with and without visibility in row 1) and row 2), respectively, for a) diffuse normal, b) specular normal, c) diffuse albedo, and d) specular albedo. Details are shown in row 3).}
    % \vspace{-10pt}
    \label{fig:visibility_improvement}
\end{figure}
% https://docs.google.com/presentation/d/15d_18Vm8ULm_pvoNpSsleL4fuM7AIQPBWvobwlRNuw4/edit?usp=sharing



==> fig/tex/rebuttal-corr.tex <==
\begin{figure}[h]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.4\linewidth]{fig/jpg/rebuttal-corr.jpg}
    \vspace{-10pt}
    \caption{Raw Capture (left) and Confidence map (right).}
    \vspace{-15pt}
    \label{fig:rebuttal-corr}
\end{figure}


==> fig/tex/rebuttal-diffuseobjects.tex <==
\begin{figure}[h]
    \centering
    \vspace{-20pt}
    \includegraphics[width=\linewidth]{fig/jpg/rebuttal-diffuseobjects.jpg}
    \vspace{-20pt}
    \caption{Diffuse Objects}
    \vspace{-15pt}
    \label{fig:rebuttal-diffuseobjects}
\end{figure}


==> fig/tex/rebuttal-interreflection.tex <==
\begin{figure}[t]
    \centering
    \vspace{-30pt}
    \includegraphics[width=\linewidth]{fig/jpg/rebuttal-interreflection.jpg}
    \vspace{-20pt}
    \caption{Inter-reflection showcase}
    \vspace{-22pt}
    \label{fig:rebuttal-interreflection}
\end{figure}


==> fig/tex/rebuttal-lightstagediffuse.tex <==
\begin{figure}[h]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.6\linewidth]{fig/jpg/rebuttal-lightstagediffuse.jpg}
    \vspace{-10pt}
    \caption{Grey ball showcase}
    \vspace{-12pt}
    \label{fig:rebuttal-lightstagediffuse}
\end{figure}


==> fig/tex/rebuttal-relighting.tex <==
\begin{figure}[h]
    \centering
    \vspace{-12pt}
    \includegraphics[width=\linewidth]{fig/jpg/rebuttal-relighting.jpg}
    \vspace{-25pt}
    \caption{Image-based Relighting. we display
the relighting results (b, d, f) alongside corresponding real captures (a, c, e)}
    \vspace{-15pt}
    \label{fig:rebuttal-relighting}
\end{figure}


==> sec/3_database.tex <==
\section{Material Database}
% \textcolor{red}{update this section as well as that in the supp}
We design our object database to span over a large variety of materials commonly found in real-world environments, such as ceramics, concrete, fur, fabrics, glass, leathers, metals, organic matter, papers, plastics, stones, terracotta, and wood. They are representative objects under our carefully defined 17 classes as shown in Fig.~\ref{fig:database} a). We captured multiview high-resolution images with high-performance cameras under varying illumination conditions for 80 different objects, enabling us to obtain detailed information over the object’s surface material convering diffuse albedo $\rho$, specular albedo $\rho_s$, roughness $\gamma$, anisotropy $\varsigma$, and surface normals $n$ and also raw images under varying illuminations. We present examples of the captured objects with obtained materials in Fig.~\ref{fig:database} (b). \textit{Details about our capture setup, and processing pipeline can be found in the supplementary material.} 
% \input{fig/tex/database}
% \input{tab/symbol}


==> sec/6_implementation.tex <==
\subsection{Implementation Details}
In our implementation, we utilized PyTorch for TexNet and MatNetwith Jax serving as the tool to accelerate the remaining components of the pipeline. The workflow for TexNet began with the synthesis of multiview images ($I_{rgb}$) at a resolution of $512 \times 512$. These images were generated from multiview renderings of various objects, conditioned on diverse prompts encompassing different categories, resulting in a total of 184,800 pairs of unwrapped images paired with material labels. The depth-to-image synthesis phase was executed using A100s and V100 GPUs, consuming a total of 205.33 GPU hours. TexNet training was carried out on 4 A100 GPUs, spanning 15,000 steps, with each step processing 16 samples at $512 \times 512$ resolution, amounting to 20 GPU hours in total. The trained Texnet can generate UV space textures at a resolution of $2048 \times 2048$, with each image requiring 40 seconds for generation on a single A100 GPU. Meanwhile, MatNet underwent training within the scope of our captured database, where each image had dimensions of $6144 \times 3240$. Material measurements across our database were conducted at the pixel level, resulting in corresponding reflectance properties at the same multiview resolution. During the training phase, we randomly sampled image patches of $512 \times 512$ resolution, acquiring the corresponding reflectance properties. Each training batch comprised 4 patches and was distributed across 4 A100 GPUs. This training process demanded a total of 666 GPU hours to achieve a well-defined material layer decomposition. 



==> tab/camera.tex <==
\begin{table}[h]
\vspace{-5pt}
\begin{center}
\begin{tabular}{lllll}
  \toprule
  Megapixel & Color Mode & Status & Resolution & Count \\ 
  \midrule
  12 & Monochrome & Polarized & $4096\times3008$ & 8 \\
  12 & RGB & Polarized & $4096\times3008$ & 8 \\
  4 & RGB & Normal & $2048\times2048$ & 9 \\
  \bottomrule
\end{tabular}
\end{center}
\caption{Camera Setup}
\label{tab:camera_setup}
\vspace{-25pt}
\end{table}

==> tab/matnet_io.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{lllll}
%       \toprule
%       Block & Type & In & Mid & Out\\ 
%       \midrule
%       Et & CLIP & 768 & - & 3 \\
%       E1 & RSU7 & 9 & 32 & 64 \\
%       E2 & RSU6 & 67 & 32 & 128 \\
%       E3 & RSU5 & 131 & 64 & 256 \\
%       E4 & RSU4 & 259 & 128 & 512 \\
%       E5 & RSU4F & 515 & 256 & 512 \\
%       E6 & RSU4F & 515 & 256 & 256 \\
%       D6 & RSU4F & 256 & 256 & 512  \\
%       D5 & RSU4F & 1027 & 256 & 512 \\
%       D4 & RSU4 & 1027 & 128 & 256 \\
%       D3 & RSU5 & 515 & 64 & 128 \\
%       D2 & RSU6 & 259 & 32 & 64 \\
%       D1 & RSU7 & 131 & 16 & 64 \\
%       \bottomrule
%     \end{tabular}
%     \caption{Blocks Details}
%     \label{tab:matnet_blocks}
% \end{table}

\begin{table*}[]
    \centering
    \begin{tabular}{llllllllllllll}
        \toprule
        Block & Et   & E1   & E2   & E3   & E4   & E5    & E6    & D6    & D5    & D4   & D3   & D2   & D1   \\
        \midrule
        Type  & CLIP & RSU7 & RSU6 & RSU5 & RSU4 & RSU4F & RSU4F & RSU4F & RSU4F & RSU4 & RSU5 & RSU6 & RSU7 \\
        In    & 768  & 9    & 67   & 131  & 259  & 515   & 515   & 256   & 1027  & 1027 & 515  & 259  & 131  \\
        Mid   & -    & 32   & 32   & 64   & 128  & 256   & 256   & 256   & 256   & 128  & 64   & 32   & 16   \\
        Out   & 3    & 64   & 128  & 256  & 512  & 512   & 256   & 512   & 512   & 256  & 128  & 64   & 64   \\
        \bottomrule
    \end{tabular}
    \caption{Blocks Details in MatNet. \textcolor{red}{to remove}}
    \label{tab:matnet_blocks}
\end{table*}
% \vspace{-10pt}

==> tab/symbol.tex <==
% \begin{table}[h]
% \vspace{-5pt}
% \begin{center}
% \small
% \begin{tabular}{llll}
%   \toprule
%   Name & Space & Symbol & Dimension\\ 
%   \midrule
%   % Vertices & World & $V$ & $\mathbb{R}^{n\times3}$ \\
%   % Vertex Normals & World & $V_n$ & $\mathbb{R}^{n\times3}$ \\
%   % Faces & World & $F$ & $\mathbb{N}_0^{m\times3}$ \\
%   % Geometry & World & $M$ & $(V,V_n,F)$ \\
%   % Depth Image & Camera & $I_d$ & $\mathbb{R}^{H_{c} \times W_{c}}$ \\
%   % Synthesis from Depth & Camera & $I_{rgb}$ & $\mathbb{R}^{H_{c} \times W_{c} \times 3}$ \\
%   % Normal Image & Camera & $I_n$ & $\mathbb{R}^{H_{c} \times W_{c} \times 3}$ \\
%   % Texture Map & UV & $T_{rgb}$ & $\mathbb{R}^{H_{uv} \times W_{uv} \times 3}$ \\
%   % Normal Map & UV & $T_n$ & $\mathbb{R}^{H_{uv} \times W_{uv} \times 3}$ \\
%   % Albedo Map & UV & $T_\rho$ & $\mathbb{R}^{H \times W \times 3}$ \\
%   % Specular Map & UV & $T_{\rho_s}$ & $\mathbb{R}^{H \times W}$ \\
%   % Roughness Map & UV & $T_{\gamma}$ & $\mathbb{R}^{H \times W}$ \\
%   % Occlusion Map & UV & $T_{\tau}$ & $\mathbb{R}^{H \times W}$ \\
%   % Anisotropy Map & UV & $T_{\varsigma}$ & $\mathbb{R}^{H \times W}$ \\
%   \bottomrule
% \end{tabular}

% \begin{tabular}{l|c|c|c|c|c}
%   % \toprule
%   Name &  Symbol &Dimension & Image Space&UV Space &Latent Space\\ 
%   \midrule
%   % Vertices & World & $V$ & $\mathbb{R}^{n\times3}$ \\
%   % Vertex Normals & World & $V_n$ & $\mathbb{R}^{n\times3}$ \\
%   % Faces & World & $F$ & $\mathbb{N}_0^{m\times3}$ \\
%   % Geometry & World & $M$ & $(V,V_n,F)$ \\
%   Depth&  d&$\mathbb{R}$& $I_d$ &- &\\
%   Color Appearance&  rgb&$\mathbb{R}^3$& $I_{rgb}$ &$\mathcal{T}_{rgb}$ &$z_{rgb}$\\
%   Diffuse Albedo&  $\rho$&$\mathbb{R}^3$& $I_\rho$&$\mathcal{T}_{\rho}$ &$z_{\rho}$\\
%   Specular Albedo&  $\rho_s$&$\mathbb{R}$& $I_{\rho_s}$&$\mathcal{T}_{\rho_s}$ &$z_{\rho_s}$\\
%   Normal&  n&$\mathbb{R}^3$& $I_n$&$\mathcal{T}_{n}$ &$z_{n}$\\
%   Occlusion&  $\tau$&$\mathbb{R}$& $I_\tau$&$\mathcal{T}_{\tau}$ &$z_{\tau}$\\
%   Roughness&  $\gamma$&$\mathbb{R}$& $I_{\gamma}$&$\mathcal{T}_{\gamma}$ &$z_{\gamma}$\\
%   Anisotropy&  $\varsigma$&$\mathbb{R}$& $I_{\varsigma}$&$\mathcal{T}_{\varsigma}$ &$z_{\varsigma}$\\
%   % \bottomrule
% \end{tabular}
% \end{center}
% \caption{Symbol table}
% \vspace{-25pt}
% \label{tab:symbol table}
% \end{table}

\begin{figure*}[tb]
  \centering
  \vspace{-5pt}
  \begin{subfigure}{0.65\linewidth}
      \begin{tabular}{clcl} 
              \hline
              I/O&Name &  Symbol&Dimension \\
              \hline
     I& Camera Pose & $\mathtt{R}, \mathtt{t}, \mathtt{K}$ &$\mathbb{R}^{3 \times 3}$, $\mathbb{R}^3$, $\mathbb{R}^{3 \times 3}$ \\ 
      I&Captured Image & $I_\perp$, $I_\parallel$&$\mathbb{R}^{H \!\times\! W \!\times\! 3}$ \\ 
      I&Captured OLAT & $\Lambda_\perp$, $\Lambda_\perp$&$\mathbb{R}^{N \!\times\! H \!\times\! W \!\times\! 3}$ \\ 
      O&Visibility Map & $\nu_d$, $\nu_s$&$\mathbb{B}^{H \!\times\! W}$ \\
     O& Occlusion Map & $\tau_d$, $\tau_s$&$\mathbb{R}_{+}^{H \!\times\! W}$ \\ 
      O&Inter-reflection Map & $\varrho_d$, $\varrho_s$&$\mathbb{R}_{+}^{H \!\times\! W \!\times\! 3}$, $\mathbb{R}_{+}^{H \!\times\! W}$ \\ 
      O&Albedo Map & $\rho_d$, $\rho_s$& $\mathbb{R}_{+}^{H \!\times\! W \!\times\! 3}$, $\mathbb{R}_{+}^{H \!\times\! W}$ \\ 
      O&Normal Map & $n_d$, $n_s$& $\mathbb{R}^{H \!\times\! W \!\times\! 3}$ \\
     O& Specular-var Map& $\sigma$&$\mathbb{R}_{+}^{H \!\times\! W \times 2}$ \\ 
      O&Anisotropy Map & $\varsigma$&$\mathbb{R}_{+}^{H \!\times\! W}$\\ 
      O&Roughness Map & $\gamma$&$\mathbb{R}_{+}^{H \!\times\! W}$ \\
    \end{tabular}
    \caption{\textbf{Symbols.} }
    \label{tab:symbols}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.34\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{fig/jpg/Polarized OLAT.jpg}
    \caption{\textbf{Polarized OLAT.}}
    \label{fig:polarized_olat}
  \end{subfigure}
  \caption{\subref{tab:symbols}. Dimensions are indicated only once if the symbols with different subscripts are within the same dimension. \subref{fig:polarized_olat} We present an object captured under the first 300 lighting conditions. The 1) row exhibits images captured through cross-polarized OLAT, while the 2) row displays parallel-polarized OLAT. In the 3) row, we zoom in on details, marked by continuous/dotted boxes, with the active light board in the lower corner accordingly. Also in the third row, we present the lighting order, progressing from blue to red, where each point represents a light board on the capture device.}
  \vspace{-10pt}
\end{figure*}
